NeuRadar: Neural Radiance Fields for Automotive Radar Point Clouds

Radar is an important sensor for autonomous driving (AD) systems due to its robustness to adverse weather and different lighting conditions. Novel view synthesis using neural radiance fields (NeRFs) has recently received considerable attention in AD due to its potential to enable efficient testing and validation but remains unexplored for radar point clouds. In this paper, we present NeuRadar, a NeRF-based model that jointly generates radar point clouds, camera images, and lidar point clouds. We explore set-based object detection methods such as DETR, and propose an encoder-based solution grounded in the NeRF geometry for improved generalizability. We propose both a deterministic and a probabilistic point cloud representation to accurately model the radar behavior, with the latter being able to capture radar's stochastic behavior. We achieve realistic reconstruction results for two automotive datasets, establishing a baseline for NeRF-based radar point cloud simulation models. In addition, we release radar data for ZOD's Sequences and Drives to enable further research in this field. To encourage further development of radar NeRFs, we release the source code for NeuRadar.

==> sec/junkyard.tex <==
\section{Introduction Stuff}

The concept of using NeRFs for novel view synthesis of Camera images was introduced in \cite{DBLP:journals/corr/abs-2003-08934}, inspiring a wave of subsequent research in various domains such as medicine \cite{9871757} or robotics \cite{9712211}. NeRFs work based on the assumption that each pixel in an image is the reflection of a ray of light originating from a camera, which goes through a scene and reflects back towards the camera. 

In \cite{yang2023unisim}, this idea is expanded to predicting multi-dimensional feature arrays $\mathbf{f} \in \mathbb{R}^N$ instead of color values, allowing the authors to use the network to generate not only images but also the Lidar point cloud, by predicting the position and intensity values of each Lidar point. This approach aligns well with how Camera and Lidar sensors capture a scene, but it doesn’t fully reflect the physical characteristics of Radar. Radar point clouds are generated through a complex signal processing chain, which results in data that is noisy and sparse compared to other sensor modalities.

Most automotive Radars are Frequency-Modulated Continuous Wave (FMCW) Radars, which operate in the frequency domain. These radars have an array of transmitter and receiver antennas in certain positions and transmit electromagnetic wave signals in regular intervals. Objects in a scene reflect this signal with a delay that is used to compute the distance and velocity of the objects relative to the sensor. The phase difference in the signal returned to the different receivers provides information on the azimuth and elevation angles. After receiving the signals, a Fast Fourier transform is required to translate the received signals back into the time domain, resulting in a multidimensional matrix called a radar cube. Each "cell" in the radar cube corresponds to a unique combination of range, azimuth, elevation, and relative radial velocity (also called range rate), encapsulating the energy level or signal intensity detected by the radar at that specific point. \cite{9369027}, \cite{srivastav2023radarsautonomousdrivingreview}, \cite{9318758}. 

The Radar point cloud with range, range rate, and angle information is obtained by extracting peaks within the radar cube using algorithms such as the constant false alarm rate (CFAR) algorithm, which classifies a cell in the radar cube as a detection point if its amplitude is larger than a certain noise threshold based on its surrounding cells \cite{9369027}, \cite{7870764}, \cite{srivastav2023radarsautonomousdrivingreview}. This leads to a loss of data richness and implies that the existence of a Radar detection for an object is dependent on objects around it and its surrounding scene, meaning that modelling a Radar detection as the reflection from a single ray projected from the sensor, similar to Camera and Lidar, is not an ideal representation of its behavior. This is the main challenge in using NeRF-based methods to render Radar data. 

Figure \ref{fig:statdet} shows radar detections from a ZOD sequence where both the ego vehicle and most surrounding objects remain stationary. By overlapping radar detections from multiple frames captured at consecutive timestamps, with ego motion compensation applied, we can clearly see slight positional variations in radar detections across frames. Each detection is color-coded to indicate its frame origin, with Lidar detections included to illustrate the true object positions.

This analysis reveals that radar detections exhibit variance across frames, even in a static environment, highlighting the advantage of using a probabilistic model to represent the radar point cloud. Such a model captures the natural dispersion in the detections' positions. Figure \ref{fig:movingdet} shows another sequence where the ego vehicle is moving. Here, with motion compensation applied, stationary objects show a slight spatial 'spread' in their radar detections across frames, further supporting the need for probabilistic modeling to achieve accurate scene representation.

\begin{figure}[ht]
    \centering
    % First subfigure
    \begin{subfigure}{0.4\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/FELV-cat.jpg}
        \caption{stationary}
        \label{fig:statdet}
    \end{subfigure}
    \hspace{0.05\textwidth} 
    % Second subfigure
    \begin{subfigure}{0.4\textwidth}
        \centering
        \includegraphics[width=\linewidth]{figures/FELV-cat.jpg}
        \caption{moving}
        \label{fig:movingdet}
    \end{subfigure}
    \caption{overlapped detections}
    \label{fig:main}
\end{figure}

Several works such as \cite{10640703} and \cite{10.1117/12.2656870} have explored neural rendering for Synthetic Aperture Radars (SAR) used for earth observation and military surveillance, which operate in a different way than automotive Radars and focus mainly on optimizing the SAR imaging process. In \cite{borts2024radarfieldsfrequencyspaceneural}, the authors directly use raw Radar data, more specifically range-azimuth heatmaps, and work in the frequency domain to reconstruct the Radar data and create a 3D representations of driving environments in the form of an occupancy map.  

However, using raw Radar data is often impractical due to high storage requirements and may not be suitable for real-world automotive applications. Processing raw radar data is more computationally intensive compared to a point cloud due to the need to handle high-dimensional data and transform them into manageable form \cite{9369027}. Point cloud is a more efficient alternative and most common automotive datasets only provide Radar point cloud data, which is why in this work, we explore the reconstruction of radar point cloud data using a NeRF-based framework capable of handling different sensor modalities from a unified representation, which adapts to any dataset. 

We use the View of Delft and nuScenes datasets, and introduce the expanded Zenseact Open Dataset, which includes Radar data in its sequences and drives. 

Our contributions are as follows.

\begin{itemize}
    \item radarnerf
    \item zod radar data
\end{itemize}

\section{Related work stuff}

Radar sensor models vary from high-fidelity, physics-based simulations that simulate radar wave propagation and complex environmental interactions \cite{10041901}, to phenomenological and probabilistic models that introduce uncertainty for an efficient approximation of the real radar output \cite{bernsteinerradar2015}, \cite{7226346}. The use of probabilistic sensor models provides a good balance between complexity and efficiency since we do not need to gather information on every detail in a scene \cite{magosi2022survey}, \cite{s24113310}, \cite{1689647}. 

\subsection{NeRFs for Radar Data}

One area of application is Synthetic Aperture Radar (SAR), where NeRF-inspired models have been used to improve 3D scene reconstruction. Traditional SAR imaging faces challenges due to the anisotropic scattering properties of radar, making it difficult to achieve consistent 3D reconstructions across different observation angles. To address this, works like SAR-NeRF and RaNeRF have been developed, which combine neural networks with SAR imaging principles to map attenuation coefficients and scattering intensities to 3D voxel grids, enabling effective 3D reconstructions from sparse SAR data, and even augmenting datasets for target classification tasks under few-shot learning scenarios (\cite{Lei2023_SAR_NeRF}, \cite{Jamora2023_SAR}, \cite{Liu2023_RaNeRF}).

Beyond SAR, a modified version of neural radiance fields have also been explored for Frequency-Modulated Continuous-Wave (FMCW) imaging radars. Radar Fields is an example of a neural method designed to work with raw frequency-domain radar data, which learns implicit scene geometry and reflectance models. By bypassing conventional volume rendering and directly modeling in frequency space, this approach manages to extract dense 3D occupancy data from 2D range-azimuth maps. This method has proven effective in urban environments, showing robustness to weather conditions where traditional optical sensors might fail (\cite{Borts2024_Radar_Fields}). 

A different direction is explored by DART (Doppler-Aided Radar Tomography), which uses radar's unique capability to measure motion through Doppler effects. DART applies a NeRF-inspired pipeline to synthesize range-Doppler images from new viewpoints, implicitly capturing the tomographic properties of radar signals. This makes it possible to reconstruct 3D radar images while accounting for object movement, which can be useful in dynamic scenarios (\cite{Huang2024_DART}). 

\subsection{Neural Rendering}

Neural Radiance Fields (NeRFs) represent a significant advancement in view synthesis by modeling complex scenes as continuous volumetric functions. Introduced by Mildenhall et al. \cite{DBLP:journals/corr/abs-2003-08934}, NeRF utilizes a fully connected Multi-Layer Perceptron (MLP) to represent a scene as a 5D continuous volumetric function. The input to the network consists of a 3D spatial location $\mathbf{x} = (x, y, z)$ and the viewing direction $\mathbf{d} = (\theta, \varphi)$, expressed as two angles. The MLP predicts two outputs: the RGB color values $\mathbf{c} = (r, g, b)$, which indicate the view-dependent radiance at that point, and a scalar density $\sigma$, which represents the differential opacity. The density $\sigma$ captures how much light is accumulated or absorbed at a specific point in space, essentially determining the likelihood of occlusion along a ray passing through $\mathbf{x}$. This enables the representation of a 3D scene as a continuous function:
\begin{equation}
    F_\Theta : (\mathbf{x}, \mathbf{d}) \rightarrow (\mathbf{c}, \sigma),
\end{equation}
where $F_\Theta$ denotes the parameters of the neural network optimized to predict accurate color and density values for novel view synthesis.

This allows for photorealistic rendering by querying points along camera rays and integrating their radiance contributions via volume rendering techniques. The process is inherently differentiable, making it possible to optimize the network by minimizing errors between the synthesized and actual images.


The publication of the original NeRF paper has led to a significant increase in research and development around neural scene representations. NeRF's ability to synthesize highly realistic novel views from sparse image data has been foundational for a range of applications, leading to advancements in dynamic scene representation (e.g., AD-NeRF for audio-driven talking head synthesis \cite{guo2021adnerf}) and more intuitive manipulation of 3D content, such as the ability to control scenes via text or images as demonstrated by CLIP-NeRF \cite{wang2022clipnerf}. Moreover, surveys such as those by Tewari et al. highlight that the field of neural rendering, propelled by NeRF, has seen hundreds of publications exploring new methods to improve speed, accuracy, and adaptability \cite{https://doi.org/10.1111/cgf.14507}.

NeRF applications have expanded beyond traditional computer graphics to fields such as cultural heritage, VR/AR environments, robotics, and medicine, showcasing its ability to adapt to diverse requirements in the capture and synthesizing of complex 3D scenes \cite{croce2023cultural}, \cite{remondino2023analysis}, \cite{9871757}, \cite{9712211}. 

NeRFs have also been extended beyond confined scenes to model large, unbounded environments, facilitating applications that require broader coverage and dynamic scene understanding. For instance, in \cite{Tancik_2022_CVPR}, a divide-and-conquer approach known as Block-NeRF was introduced, which divides expansive areas into smaller, overlapping blocks, each represented by a separate NeRF. This method enables scalable modeling of extensive regions, such as urban landscapes, while maintaining manageable computational requirements. Additionally, works like \cite{Martin-Brualla_2021_CVPR} explored separating the dynamic and static components of a scene into distinct NeRFs. This approach allows the dynamic part to capture non-static elements, overcoming the traditional NeRF assumption that density remains constant, making it possible to render scenes with changing elements such as moving cars or people. Another important advancement is presented in \cite{Ost_2021_CVPR}, where neural scene graphs were utilized to represent dynamic environments, further enhancing the ability of NeRFs to adapt to changes within a scene. 

\subsection{NeRFs for Autonomous Driving}

NeRF-based models can reconstruct high-fidelity 3D scenes from multiview images, allowing autonomous systems to create detailed maps of their surroundings. This is crucial for navigation and planning, as it helps vehicles better understand complex environments, especially in urban areas where accurate 3D information is essential for safe navigation \cite{10.1007/978-981-99-8850-1_1}, \cite{yang2023unisim}, \cite{tonderski2023neurad}. 

MARS focuses on modularity by decomposing driving environments into manageable static and dynamic components, allowing detailed control over individual elements in a scene. This instance-aware approach improves scalability and real-time interaction, making it effective for large-scale driving scenarios \cite{10.1007/978-981-99-8850-1_1}. UniSim extends these capabilities by integrating Lidar modeling and simulating realistic interactions between dynamic objects in the scene and their environment \cite{yang2023unisim}. NeuRAD further incorporates sensor-specific details such as ray drop and beam divergence for Lidar, which helps close the gap between simulated and real-world data \cite{tonderski2023neurad}. 

Building on the versatility of NeRFs for autonomous driving, these methods have extended the concept to Neural Feature Fields (NFFs), which allow for a broader range of outputs beyond simple RGB colors. NFFs predict feature arrays, enabling the representation of various attributes such as texture, geometry, and sensor-specific data. 

NFFs work by mapping a 3D spatial location $\mathbf{x}$ and a viewing direction $\mathbf{d}$ to a multidimensional feature vector $\mathbf{f}$ instead of RGB values. The feature vector is computed by volume rendering, which accumulates the features at sampled points along a ray $\mathbf{r}$. This process can be expressed as follows:

\begin{equation}
    \mathbf{f}(\mathbf{r}) = \sum_{i = 1}^{N_\mathbf{r}} \omega_i \mathbf{f}_i, \,\,\,\, \omega_i = \alpha_i \prod_{j = 1}^{i - 1} (1 - \alpha_j),
    \label{eq:volrenfeature}
\end{equation}

where $\mathbf{f}_i$ is the feature value at the $i$-th sample point, $\alpha_i$ denotes the opacity at that point and $\omega_i$ determines the contribution of each feature along the ray, which is based on the density values predicted by the NFF. These feature values can then be decoded into the desired sensor-specific features using an appropriate network architecture, such as a Convolutional Neural Network (CNN) or MLP. 

In NeuRAD, NFFs are instrumental in simulating sensor data by capturing detailed sensor characteristics, such as Lidar-specific effects like ray drop and beam divergence \cite{tonderski2023neurad}. In this work, the NFF architecture in NeuRAD is used to also generate radar point cloud data.

\subsection{Random Finite Sets}

A Bernoulli process is an RFS which has the distribution:

\begin{equation}
    f(\textbf{X}) = \begin{cases}
    1-r, & \textbf{X} = \emptyset \\
    rf(\textbf{x}), & \textbf{X} = \{\textbf{x}\} \\
    0, & |\textbf{X}| \geq 2
  \end{cases} \, ,
    \label{eq:bp}
\end{equation}

where $r$ is the probability of existence and $f(\textbf{x})$ is the existence-conditioned probability density function of a single element. In this work each Bernoulli represents one Radar point in a point cloud. The point cloud itsel is represented as a Multi-Bernoulli (MB).

The Multi-Bernoulli density for a set \textbf{X} is represented as

\begin{equation}
    f(\textbf{X}) = \begin{cases}
    \sum_{\uplus_{i\in \mathbb{I}} \textbf{X}^i = \textbf{X}} \prod_{i\in \mathbb{I}}f^i\textbf{X}^i, & |\textbf{X}| \leq |\mathbb{I}| \\
    0, & |\textbf{X}| > |\mathbb{I}|
  \end{cases} \; ,
    \label{eq:mbp}
\end{equation}

where $\mathbb{I}$ is the index set of all the Bernoullis in the Multi-Bernoulli and $\textbf{X}$ is a union of a fixed number of independent Bernoulli RFSs $\textbf{X}^i$ where $\textbf{X}^i \cap \textbf{X}^j = \emptyset$, $i, \,j \in \mathds{I}$ and $\textbf{X} = \cup_{i\in\mathds{I}} \textbf{X}^i$.

\section{method stuff}

\begin{comment}

\subsubsection{Range Rate}
\label{sec:rangerate}

To predict the radial velocities of objects towards the sensor, we use the velocity information from the ego vehicle and the annotations and create a velocity hashgrid which can be used to render radial velocity features, similar to the NFF features. 
\\
One of the advantages of Radar is that it can measure the velocity of an object relative to the sensor, which is also called range rate. In order to also generate the range rate of the detections, we need to have some information about the velocity of the objects in the scene around us. Unfortunately we don't have that information. There only info that we have or can derive is the velocity of the annotated objects in a sequence. We already use the annotated objects in the neural feature field to create separate hashgrids for the static scene and dynamic objects. We can use this logic alongside the velocity information from the annotations and the assumption that the velocity of all objects in the static scene is zero to generate range rate values for the Radar detections. This is done in a similar process to volume rendering the features. We assign a velocity relative to the Radar sensor to each sample along the Radar ray, so each sample will have it's own range rate. If the ego vehicle (or Radar sensor) moves with velocity $\upsilon_{e}$, the range rate of the samples in the static scene will be equal to $-d^T \upsilon_{e}$. In that case, the velocity of samples from the dynamic actors relative to the ego vehicle is equal to $d^T (\upsilon_{object} - \upsilon_{e})$. Whether a sample is static or dynamic depends on the position of the sample in the scene.

These range rate values are then encoded using an MLP to generate velocity features, which are arrays similar to the feature arrays from the NFF. We can then find the velocity feature array for each ray using volume rendering, which can be seen as a weighted sum of velocity features along a ray where the weights are dependant on the predicted density or geometry info from the NFF. The per ray velocity features can then be added to or concatenated with the NFF features. In our experiments we have added the two features. 

\begin{equation}
    \mathbf{f}(\mathbf{r}) = \sum_{i = 1}^{N_\mathbf{r}} \omega_i \mathbf{f}_i,\,\,\,\, \omega_i = \alpha_i \prod_{j = 1}^{i - 1} (1 - \alpha_j)
\end{equation}

\begin{equation}
    \mathbf{\upsilon}(\mathbf{r}) = \sum_{i = 1}^{N_\mathbf{r}} \omega_i \mathbf{\upsilon}_i
\end{equation}

This will give the network some info about the velocity, but this is not enough information to predict the range rate from, so the range rate values are estimated in a probabilistic manner similar to other Radar features such as range and azimuth. 

\end{comment}


\begin{comment}

The volumetric rendering process results in a sequence of arrays with shape $(N_\phi N_\theta) \times N_{\mathbf{f}}$. These features are then fed to a Radar decoder unit, which consists of a transformer and MLPs which decode the transformer output to get a set prediction of all possible Radar detections, inspired by \cite{Hess_2022}, where the prediction is modelled as an RFS and the output from an object detection network is represented as a Poisson Multi-Bernoulli distribution. We can then find the best assignment between the predicted Bernoullis and ground truth to compute the negative log likelihood of the Multi-Bernoulli, which is added to the total training losses. 


To obtain the probabilistic representation of the Radar point cloud, we use a transformer decoder layer. The transformer queries have the shape $m \times N_\mathbf{f}$, where m is the number of predictions which represents the number of expected Radar detection points. 

\end{comment}

Log prob for Guassians (to demonstrate the effect of scaling the azimuth and elevation values and not necessarily for paper):

\begin{align}
    &\log(p(x)) = \log(\frac{1}{\sigma \sqrt{2\pi}}\exp(-\frac{1}{2}(\frac{x - \mu}{\sigma})^{2}))\\
    &=-\log(\sigma)-\log(\sqrt{2\pi})-\frac{1}{2}(\frac{x - \mu}{\sigma})^{2}
    \label{eq:guassianlogprob}
\end{align}




The Chamfer distance

GOSPA is a measure of similarity between two finite sets. In this context, the GOSPA metric considers both the euclidean distance between the prediction and the ground truth but also the missed predictions and the false detections. Assuming that $X = \{x_1, \dots, x_{|X|}\}$ and $Y = \{y_1, \dots, y_{|Y|}\}$ are finite subsets of $\mathbb{R}^N$ such that $|X| \leq |Y|$, GOSPA is defined as:

\begin{align}
    d^{c, \alpha}_p \triangleq \Bigg{(} \min_{\pi \in \Pi_{|Y|}} \sum_{i=1}^{|X|} d^{(c)}(x_i, y_{\pi(i)})^p + \frac{c^p}{\alpha}(|Y| - |X|) \Bigg{)}^{\frac{1}{p}}, 
\end{align}

where $d(x, y)$ is a metric for any $x, y, \in \mathbb{R}^n$ with cut-off metric $d^{(c)}(x, y) = \min(d(x, y), c)$ and $\Pi_n$ is a set of all permutations of $\{ 1, \dots,n \}$ for any $n\in \mathbb{N}$, each element of which $\pi \in \Pi_n$ is a sequence $\pi = (\pi(1), \dots, \pi(n))$. The parameter $c > 0$ determines the maximum allowable localization error and contributes to the cost for the difference in set cardinalities, alongside the parameter $0 < \alpha \leq 2$. The parameter $1 \leq p < \infty$ determines how much outliers are penalized. Here, the GOSPA is calculated with parameters $\alpha = 2$, $c = 1$, and $p = 1$ and $d(x, y)$ is the euclidean distance between two Radar detections. With $\alpha = 2$, GOSPA can be expressed as an optimization over assignment sets, so the definition can be written as:

\begin{align}
    &d^{1, 2}_1 \triangleq \Bigg{(} \min_{\gamma \in \Gamma} \sum_{i, j \in \gamma}^{|X|} d^{(1)}(x_i, y_j) \\
    &+ \frac{1}{2}(\underbrace{|Y| - |\gamma |}_{\# missed\,predictions} + \underbrace{|X| - |\gamma |}_{\# false\,predictions}) \Bigg{)}
\end{align}

where $\Gamma$ is the set of all possible assignment sets $\gamma$. 


